Sparse Probability of Agreement

Measuring inter-annotator agreement is important for annotation tasks, but many metrics require a fully-annotated set of data, where all annotators annotate all samples. We define Sparse Probability of Agreement, SPA, which estimates the probability of agreement when not all annotator-item-pairs are available. We show that under certain conditions, SPA is an unbiased estimator, and we provide multiple weighing schemes for handling data with various degrees of annotation.

==> resources/dtu_colors.tex <==
 %%%%
 % DTU colors
 
\definecolor{DTURed}{cmyk}{0, 0.91, 0.72, 0.23}
\definecolor{DTUGray}{cmyk}{0, 0, 0, 0.56}

\definecolor{DTU_sek_1}{cmyk}{0, 0.5, 1.0, 0} % Orange
\definecolor{DTU_sek_2}{cmyk}{0, 0.75, 1.0, 0} % Orage-red
\definecolor{DTU_sek_3}{cmyk}{0, 1, 1, 0} % Red
\definecolor{DTU_sek_4}{cmyk}{0, 1, 1, 0.5} % Dark-red
\definecolor{DTU_sek_5}{cmyk}{0, 1, 0, 0} % Light pink
\definecolor{DTU_sek_6}{cmyk}{0.25, 1, 0, 0} % Pink
\definecolor{DTU_sek_7}{cmyk}{0.5, 1, 0, 0} % Purple
\definecolor{DTU_sek_8}{cmyk}{0.75, 1, 0, 0} % Purple-blue
\definecolor{DTU_sek_9}{cmyk}{0.75, 0.75, 0, 0} % Blue
\definecolor{DTU_sek_10}{cmyk}{0.5, 0, 0, 0} % Turqoise
\definecolor{DTU_sek_11}{cmyk}{0.25, 0, 1, 0} % Green-yellow
\definecolor{DTU_sek_12}{cmyk}{0, 0.25, 1.0, 0} % Yellow
\definecolor{DTU_sek_13}{cmyk}{0.75, 0.5, 0, 0} % Light-blue
\definecolor{DTU_sek_14}{cmyk}{0.5, 0, 1, 0} % Green

\colorlet{DTU_sek_orange}{DTU_sek_1}
\colorlet{DTU_sek_orange_red}{DTU_sek_2}
\colorlet{DTU_sek_red}{DTU_sek_3}
\colorlet{DTU_sek_dark_red}{DTU_sek_4}
\colorlet{DTU_sek_light_pink}{DTU_sek_5}
\colorlet{DTU_sek_pink}{DTU_sek_6}
\colorlet{DTU_sek_purple}{DTU_sek_7}
\colorlet{DTU_sek_purple_blue}{DTU_sek_8}
\colorlet{DTU_sek_blue}{DTU_sek_9}
\colorlet{DTU_sek_turqoise}{DTU_sek_10}
\colorlet{DTU_sek_green_yellow}{DTU_sek_11}
\colorlet{DTU_sek_yellow}{DTU_sek_12}
\colorlet{DTU_sek_light_blue}{DTU_sek_13}
\colorlet{DTU_sek_green}{DTU_sek_14}

==> resources/expand_in_lstlistings.tex <==
\RequirePackage{listings}
% From: https://tex.stackexchange.com/questions/487769/expand-macro-inside-lstlisting-and-apply-syntax-highlighting

\makeatletter
\gdef\lst@CSEscape#1{%
    \lst@CArgX #1\relax\lst@CDefX
        {}%
        {\lst@ifdropinput\else
         \lst@TrackNewLines\lst@OutputLostSpace \lst@XPrintToken
         \lst@InterruptModes
         \lst@EnterMode{\lst@TeXmode}{\lst@modetrue}%
         \let\do\@makeother\dospecials
         \let\lst@grabbed@csname\@empty
         \expandafter\lst@scan@csname%
         \fi}%
        {}}
\lst@Key{cschar}{}
    {\ifx\@empty#1\@empty
       \let\lst@CSChar\relax
     \else
       \def\lst@CSChar{\lst@CSEscape{#1}}%
     \fi}
\let\lst@explicit@space=\ %
\lst@AddToHook{SelectCharTable}{\lst@CSChar}
\def\lst@afterfi#1#2\fi{\fi#1}
\def\lst@scan@csname#1{%
  \if\relax\detokenize{#1}\relax
    \lst@afterfi{\lst@dispatch@csname{#1}}%
  \else
    \lst@afterfi{%
      \uppercase{\def\lst@tmpa{#1}}%
      \expandafter\lst@scan@csname@\expandafter
        {\number\expandafter`\lst@tmpa}{#1}}%
  \fi}
\def\lst@scan@csname@#1#2{%
  \ifnum %      vv If you want to \maketatletter :)
    % \ifnum0#1>63 \expandafter0\else\expandafter1\fi
      \ifnum0#1>64 \expandafter0\else\expandafter1\fi
      \ifnum0#1<91 \expandafter0\else\expandafter1\fi
        =0
    \edef\lst@grabbed@csname{\lst@grabbed@csname\string#2}%
    \expandafter\lst@scan@csname
  \else
    \lst@afterfi{\lst@dispatch@csname{#2}}%
  \fi}
\def\lst@dispatch@csname#1{%
  \ifx\lst@grabbed@csname\@empty
    \if\detokenize{#1}\lst@char@space
      \lst@afterfi{\lst@afterfi{\lst@return@from@csname@{}{#1}}}%
    \else
      \lst@afterfi{\lst@afterfi{\lst@dispatch@csname@{\string#1}}}%
    \fi
  \else
    \lst@afterfi{\expandafter\lst@dispatch@csname@\expandafter{\lst@grabbed@csname}{#1}}%
  \fi}
\def\lst@dispatch@csname@#1{%
  \@ifundefined{#1}%
    {\PackageError{Listings}{! Undefined control sequence \@backslashchar#1}}%
    {\expandafter\lst@return@from@csname\csname#1\endcsname}}
\def\lst@return@from@csname#1{%
  \ifx#1\lst@explicit@space
    \lst@afterfi{\lst@return@from@csname@{}{}}%
  \else
    \lst@afterfi{\expandafter\lst@return@from@csname@\expandafter{#1}}%
  \fi}
\def\lst@return@from@csname@#1#2{%
  \lst@escapeend \lst@LeaveAllModes\lst@ReenterModes
  \lst@newlines\z@ \lst@whitespacefalse
  \lst@csescape@output{#1}{#2}}
\def\if@single@item#1{%
  \if\relax\detokenize\expandafter{\@gobble#1}\relax
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondofone
  \fi}
\def\lst@active@space{\lst@ProcessSpace}
\begingroup
\catcode`\|=0
\catcode`\[=1
\catcode`\]=2
\let\do\@makeother\dospecials
[|global|let|lst@char@space= ]
|endgroup
\def\lst@csescape@output#1#2{%
  \if@single@item{#2}%
    {%
      \ifnum
        \ifx\lst@active@space#2\expandafter1\else\expandafter0\fi
        \ifx\lst@char@space#2\expandafter1\else\expandafter0\fi
        >0
        \def\lst@aftertokens{\safescantokens{#1}\lst@ProcessSpace}%
      \else
        \def\lst@aftertokens{\safescantokens{#1#2}}%
      \fi
    }{%
      \def\lst@aftertokens{\safescantokens{#1#2}}%
    }%
  \lst@aftertokens
}
\makeatother
\ExplSyntaxOn
\cs_new_protected:Npn \safescantokens #1 { \tl_rescan:nn {} {#1}}
\ExplSyntaxOff

\lstdefinestyle{expandable}{cschar=\\, basicstyle=\ttfamily}



==> resources/math_notation/print_math.tex <==
\clearpage
\section{Mathematical Notation}
\vspace{0.5cm}
\newboolean{showcode}
\setboolean{showcode}{true}

\newcommand{\showcode}[1]{
	\ifthenelse{\boolean{showcode}}{ {#1} }{}
}

\subsection*{Numbers and Arrays}





{
\def\arraystretch{1.5}
\begin{tabular}{p{2.5cm}p{3.8cm}p{11cm}}
	$\displaystyle a, \theta$           & \verb+a, \theta+           & A scalar (integer or real)                             \\
	$\displaystyle \va, \vtheta, \vone$ & \verb+\va, \vtheta, \vone+ & A vector                                               \\
	$\displaystyle \mA, \mTheta$        & \verb+\mA, \mTheta+        & A matrix                                               \\
	$\displaystyle \tA$                 & \verb+\tA+                 & A tensor                                               \\
	$\displaystyle \mI_n$               & \verb+\mI_n+               & Identity matrix with $n$ rows and $n$ columns          \\
	$\displaystyle \mI$                 & \verb+\mI+                 & Identity matrix with dimensionality implied by context \\
	$\displaystyle \ra$                 & \verb+\ra+                 & A scalar random variable                               \\
	$\displaystyle \rva$                & \verb+\rva+                & A vector-valued random variable                        \\
	$\displaystyle \rmA$                & \verb+\rmA+                & A matrix-valued random variable
\end{tabular}
}
\vspace{0.25cm}


\subsection*{Indexing}
{
\def\arraystretch{1.5}
\begin{tabular}{p{2cm}p{5.8cm}p{11cm}}
	$\displaystyle \eva_i, \evtheta_i$         & \verb+\eva_i, \evtheta_i+         & Element $i$ of vector $\va$                           \\
	$\displaystyle \eva_{-i}$                  & \verb+\eva_{-i}+                  & Element $n-i+1$ of vector $\va$ (-1 for last element) \\
	$\displaystyle \emA_{i,j}, \emTheta_{i,j}$ & \verb+\emA_{i,j}, \emTheta_{i,j}+ & Element $i, j$ of matrix                              \\
	$\displaystyle \mA_{i,:}, \emTheta_{i,:}$  & \verb+\mA_{i, :}, \emTheta_{i,:}+ & Row $i$ of matrix                                     \\
	$\displaystyle \mA_{:,i}, \emTheta_{:,i}$  & \verb+\mA_{:, i}, \emTheta_{:,i}+ & Column $i$ of matrix                                  \\
	$\displaystyle \etA_{i, j, k}$             & \verb+\etA_{i, j, k}+             & Element $(i, j, k)$ of a 3-D tensor                   \\
	$\displaystyle \tA_{:, :, i}$              & \verb+\tA_{:, :, i}+              & 2-D slice of a 3-D tensor                             \\
	$\displaystyle \erva_i$                    & \verb+\erva_i+                    & Element $i$ of the random vector                      \\
	$\displaystyle \ermA_i$                    & \verb+\ermA_i+                    & Element $i$ of the random matrix
\end{tabular}
}
\vspace{0.25cm}


\subsection*{Sets}
{
\def\arraystretch{1.5}
\begin{tabular}{p{2.5cm}p{3.8cm}p{11cm}}
	$\displaystyle \sA$                 & \verb+\sA+                & A set                                             \\
	$\displaystyle \R, \N, \Z, \Q$      & \verb+\R, \N, \Z, \Q+     & Standard sets                                     \\
	$\displaystyle \{0, 1\}$            & \verb+\{0, 1\}+           & The set containing 0 and 1                        \\
	$\displaystyle \{0, 1, \dots, n \}$ & \verb+\{0, 1, \dots, n\}+ & The set of all integers between $0$ and $n$       \\
	$\displaystyle [a, b]$              & \verb+[a, b]+             & The real interval including $a$ and $b$           \\
	$\displaystyle (a, b]$              & \verb+(a, b]+             & The real interval excluding $a$ but including $b$
\end{tabular}
\vspace{0.25cm}
}


\subsection*{Calculus}
\def\arraystretch{1.5}
\begin{tabular}{p{2.5cm}p{3.8cm}p{11cm}}
	$\displaystyle \diff[x]{y}$        & \verb+\diff[x]{y}+      & Derivative of $y$ with respect to $x$                      \\[2ex]
	$\displaystyle \pardiff[x]{y} $    & \verb+\pardiff[x]{y}+   & Partial derivative of $y$ with respect to $x$              \\
	$\displaystyle \gradient{x}y $     & \verb+\gradient{x}y+    & Gradient of $y$ with respect to $\vx$                      \\
	$\displaystyle \mdiff[\mX]y $      & \verb+\mdiff[\mX]y+     & Matrix derivatives of $y$ with respect to $\mX$            \\
	$\displaystyle \tdiff[\tX]y $      & \verb+\tdiff[\tX]y+     & Tensor containing derivatives of $y$ with respect to $\tX$ \\
	$\displaystyle \hess[\vx]f(\vx)$   & \verb+\hess[\vx]f(\vx)+ & The Hessian matrix of $f$ at input point $\vx$             \\
	$\displaystyle \int f(\vx) \d\vx $ & \verb+\int f(\vx)\d\vx+ & Definite integral over the entire domain of $\vx$
\end{tabular}
\vspace{0.25cm}

\subsection*{Probability and Information Theory}
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
	$\displaystyle P(\ra)$                                      & A probability distribution over a discrete variable                                                          \\
	$\displaystyle p(\ra)$                                      & A probability distribution over a continuous variable, or over a variable whose type has not been specified  \\
	$\displaystyle \ra \sim P$                                  & Random variable $\ra$ has distribution $P$                                                                   \\
	$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$                                                               \\
	$\displaystyle \var(f(x)) $                                 & Variance of $f(x)$ under $P(\rx)$                                                                            \\
	$\displaystyle \cov(f(x),g(x)) $                            & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$                                                               \\
	$\displaystyle H(\rx) $                                     & Shannon entropy of the random variable $\rx$                                                                 \\
	$\displaystyle \KL ( P \Vert Q ) $                          & Kullback-Leibler divergence of P and Q                                                                       \\
	$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$         & Gaussian distribution %
	over $\vx$ with mean $\vmu$ and covariance $\mSigma$
\end{tabular}
\vspace{0.25cm}

\subsection*{Functions}
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
	$\displaystyle f: \sA \rightarrow \sB$     & The function $f$ with domain $\sA$ and range $\sB$                                                                                \\
	$\displaystyle f \circ g $                 & Composition of the functions $f$ and $g$                                                                                          \\
	$\displaystyle f(\vx ; \vtheta) $          & A function of $\vx$ parametrized by $\vtheta$.	(Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation)  \\
	$\displaystyle \log x$                     & Natural logarithm of $x$                                                                                                          \\
	$\displaystyle \sigma(x)$                  & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$                                                                         \\
	$\displaystyle \zeta(x)$                   & Softplus, $\log(1 + \exp(x))$                                                                                                     \\
	$\displaystyle || \vx ||_p $               & $p$ norm of $\vx$                                                                                                                 \\
	$\displaystyle || \vx || $                 & $2$ norm of $\vx$                                                                                                                 \\
	$\displaystyle x^+$                        & Positive part of $x$, i.e., $\max(0,x)$                                                                                           \\
	$\displaystyle \vone_{\mathrm{condition}}$ & is 1 if the condition is true, 0 otherwise
\end{tabular}
\vspace{0.25cm}

==> tex/a_different_formulation.tex <==


\clearpage
\section{A different formulation}

\subsection{Annotation Tensor}

We consider an annotation task, and define the following annotation tensor $\I$, which is essentially an indicator function
\begin{align}
	&\I \in \{0, 1\}^{W \times I \times C}, \\
	&\I_{wic} = \begin{cases}
		1 & \text{worker $w$ annotated item $i$ as class $c$} \\
		0 & \text{otherwise},
	\end{cases} \nonumber
\end{align}
where $W$ is the number of workers, $I$ is the number of items, $C$ is the number of classes/labels and $I_{wic}$ indicates whether worker $w$ annotated item $i$ with class $c$. We consider classification problems (and not multi-labelling problems) so that a worker assigns at most one class to an item
\begin{align}
	\forall i, w \quad \sum_c \I_{wic} \in \{0, 1\}.
\end{align}

With the shorthand notations shown in table \ref{tbl:shorthand_notation_and_I} we can compute Fleiss kappa and other measures. \\
\begin{table}[t]
	\renewcommand{\arraystretch}{1.3}
	\caption{Shorthand notations and their relation to annotation tensor $\I$. \# denotes 'number of annotations'.} \label{tbl:shorthand_notation_and_I}
	\begin{tabular}{lL{m}{4.4cm}}
		$n = \sum_{wic} \I_{wic}$ & total \# \\
		$n_i = \sum_{wc} \I_{wic}$ & \# for item $i$ \\
		$n_c = \sum_{wi} \I_{wic}$ & \# into class $c$ \\
		$n_w = \sum_{ic} \I_{wic}$ & \# made by worker $w$ \\
		$\I_{wi} = \sum_{c} \I_{wic}$ & indicates whether worker $w$ annotated item $i$ \\
		$n_{wc} = \sum_{i} \I_{wic}$ & \# from worker $w$ into class $c$ \\
		$n_{ic} = \sum_{w} \I_{wic}$ & \# of item $i$ into class $c$
	\end{tabular}
\end{table}

We can represent missing/unfinished annotations by creating an additional indicator matrix
\begin{align}
	&\J \in \{0, 1\}^{W \times I} \\
	&\J_{wi} = \begin{cases}
		1 & \text{$w$'s annotation of $i$ is available} \\
		0 & \text{otherwise}.
	\end{cases} \nonumber \\
	&\I = \I_{\text{full}} \otimes \J,
\end{align}
where $\I_{\text{full}}$ is the (hypothetical) full annotation dataset between all workers and items, $\I$ is the available annotation tensor, and $\otimes$ is element-wise product which is broadcasted across the class dimension $c$.


\subsection{Annotation Agreement and Chance Correction}

The most intuitive way of representing agreement on a task is the following: if we pick two random workers and a random item, what is the probability that the workers will agree on that item. We represent this probability by
\begin{align*}
	&P = p\Big(f_{w_1}(i) = f_{w_2}(i)\Big), \\ 
	&w_1, w_2 \sim p_{\mathcal{W}} \qquad i \sim p_{\mathcal{I}},
\end{align*}
where $f_w(i)$ represents the (stochastic) labelling process of worker $w$ on item $i$, $p_{\mathcal{W}}$ is the probability distribution across workers and $p_{\mathcal{I}}$ is the probability distribution across items. However, this measure is not always easy to analyse or compare, because there can be a large agreement-by-chance. Problems with large majority class for example, will have very large probability of agreeing from simply guessing the majority class. \\

Therefore a commonly used measurement is the chance-corrected probability of agreement, called Fleiss kappa,
\begin{align}
	\kappa &= \frac{P - P_e}{1 - P_e} \label{eq:fleiss_formulation_1} \\
		&= \frac{1 - 1 + P - P_e}{1 - P_e} \nonumber \\
		&= \frac{1 - P_e}{1 - P_e} + \frac{P - 1}{1 - P_e} \nonumber \\
		&= 1 - \frac{1 - P}{1 - P_e}, \label{eq:fleiss_formulation_2}
\end{align}
where (\ref{eq:fleiss_formulation_1}) and (\ref{eq:fleiss_formulation_2}) are both common formulations and $P_e$ is the expected agreement-by-chance.\\

We usually do not have access to neither $P$ nor $P_e$ and will estimate them based on data by
\begin{align}
	\bar{P} &= \frac{1}{I} \sum_i \bar{P}_i 
	= \frac{1}{I} \sum_i \sum_c \frac{n_{ic}^{\mathcal{D}} (n_{ic}^{\mathcal{D}} - 1)}{2} \\
	\bar{P_e} &= \sum_c \left( \frac{n_c^{\mathcal{T}}}{n^{\mathcal{T}}} \right)^2,
\end{align}
where $\mathcal{D}$ and $\mathcal{T}$ are two datasets. \\

When computing $\bar{P}$ and $\bar{P_e}$, we often use the same datasets for the two approximations $\mathcal{D} = \mathcal{T}$. 
This makes the fraction in (\ref{eq:fleiss_formulation_2}) a \textit{ratio estimator}, which approximates the mean ratio of two random variables by the ratio of their means. Ratio estimators are biased estimators due to Jensen's inequality. 
The bias of ratio estimators are known to be on the order of $O(1/n)$, and so the bias will be small for large datasets. 


\subsection{Rewriting Kappa}

We rewrite the formulation of kappa by
\begin{align}
	\kappa &= 1 - \frac{1 - \bar{P}}{1 - \bar{P}_e}
		= 1 - \frac{1 - \frac{1}{I} \sum_i^I \bar{P}_i}{1 - \bar{P}_e} \nonumber \\
		&= 1 - \frac{I - \sum_i^I \bar{P}_i}{I(1 - \bar{P}_e)} 
		= 1 - \frac{1}{I} \frac{\sum_i^I (1 - \bar{P}_i)}{1 - \bar{P}_e} \nonumber \\
		&= 1 - \frac{1}{I} \sum_i^I \frac{1 - \bar{P}_i}{1 - \bar{P}_e}.
%		&= 1 - \frac{1}{1 - \bar{P}_e} + \frac{1}{1 - \bar{P}_e}\bar{P} \nonumber \\
%		&= 1 - \frac{1}{1 - \bar{P}_e} \nonumber \\
%		&\quad + \frac{1}{I(1 - \bar{P}_e)} \sum_i^I P_i \nonumber \\
%		&= 1 - \frac{1}{1 - \bar{P}_e} \nonumber \\
%		&\quad + \frac{1}{I(1 - \bar{P}_e)n(n-1)} \sum_{ic} n_{ic}(n_{ic} - 1) \nonumber
\end{align}

Fleiss kappa can therefore also be considered 1 minus the mean, chance-corrected disagreement of individual items (disagreement being 1 minus agreement and vice versa). 

\subsection[Alternative measure: tau]{Alternative measure: $\tau$}

We now introduce an alternative measure $\tau$, where we chance-correct the agreement on each item $i \in \mathcal{D}$, using the leave-one-out dataset $\mathcal{D} \setdiff i$
\begin{align}
	\tau &= 1 - \frac{1}{I} \sum_{i \in \mathcal{D}} \frac{1 - \bar{P}_i}{1 - \bar{P}_{e, \mathcal{D} \setdiff i}(i)}.
\end{align}
If the dataset is sampled iid. then $\bar{P}$ and $\bar{P}_{e, \mathcal{D} \setdiff i}(i)$ are statistically independent, making each fraction an unbiased estimator of the chance-corrected disagreement of the item. This in turn makes the right-side term an unbiased estimator of the mean disagreement, and gets rid of the bias mentioned earlier. 

\subsection{Probability of Agreement on Item}

Following the ideas from Fleiss kappa, one way to approximate the expected agreement on item $i$ is 
\begin{align}
	\bar{P}_{e, \mathcal{D} \setdiff i}(i)
		&= \sum_c p_{c, \mathcal{D} \setdiff i}(i)^2 \\
		p_{c, \mathcal{D} \setdiff i}(i) &= \frac{n_c - n_{ic}}{n - n_i},
\end{align}
which uses the global leave-one-item-out class-distributions. \\

This works well, when all workers annotate all items, as the leave-one-item-out class-distributions will approximate the global class-distribution arbitrarily well with large datasets. \\

In the case where our annotation tensor $\I$ has been manipulated by some availability tensor $\J$, each item is seen by a different set of workers. For a homogeneous worker-base, thi remain unproblematic, as the global class-distribution will approximate the class-distribution of the workers as well. However, for heterogeneous worker-bases (some workers act significantly differently from others), this is no longer the case. One item could randomly be assigned a group of heterogeneous workers (with low agreement), while another item may be assigned a group of homogeneous workers (with high agreement). \\

We therefore look at the case of two workers $w_1$ and $w_2$ annotating item $i$, and wish to approximate the probability
\begin{align}
	p\Big(f_{w_1}(i) = f_{w_2}(i)\Big),
\end{align}
based on class-distributions. \\

The class-distribution for a worker $w$, when ignoring item $i$, can be empirically approximated by
\begin{align}
	p_c(w) \approx \frac{n_{wc} - \I_{wic}}{n_{w} - \I_{wi}}.
\end{align}

This distribution will, however, have extreme properties for workers with few annotations, as some classes will be assigned probability zero. Using the Bayesian approach of assigning the conjugate (Dirichlet) prior to the categorical distribution, we have the following alternative approximation
\begin{align}
	p_c(w) &\approx \frac{n_{wc} - \I_{wic} + \lambda \evalpha_c}{n_{w} - \I_{wi} + \lambda} \\
	\valpha^{\top} \vone &= 1,
\end{align}
where $\lambda \alpha_c$ can be interpreted as "observed data in class $c$ available before applying the data" and $\lambda$ is a factor here used to control the importance of the prior, while $\alpha$ determines the shape of the prior. A suitable $\alpha$ to use could be the class-distribution computed from some independent set of workers and items. When determining the expected agreement of workers $w_1$ and $w_2$ on item $i$, we therefore use the class-distribution determined empirically from the worker set $\mathcal{W}\setdiff \{w_1, w_2\}$, when ignoring item $i$
\begin{align}
	&p_{w_1 \given w_2, i}(c) \approx \frac{n_{w_1c} - \I_{w_1ic} + \lambda \evalpha_{w_1, w_2, i}(c)}{n_{w_1} - \I_{w_1i} + \lambda} \nonumber \\
	&\evalpha_{w_1, w_2, i}(c) \nonumber \\
	&\:\: = \frac{ n_c - n_{w_1c} - n_{w_2c} - n_{ic} + \I_{w_1ic} + \I_{w_2ic}}{ n - n_{w_1} - n_{w_2} - n_i + \I_{w_1i} + \I_{w_2i}} \nonumber \\
	&P_{w_1, w_2}(i) = \sum_c p_{w_1 \given w_2, i}(c) p_{w_2 \given w_1, i}(c).
\end{align}

We recommend setting $\lambda \geq C$, so that workers' class-distributions stays relatively flat, until they have a chance to distribute annotations between multiple classes. 
We note that for large datasets and large $\lambda$, we have
\begin{align}
	\lim_{n, \lambda \rightarrow \infty} p_c(w_1 \given w_2, i) \rightarrow p_c,
\end{align}
where $p_c$ is the true class distribution. This makes the overall measurement
\begin{align}
	\lim_{n, \lambda \rightarrow \infty} \tau \rightarrow \kappa.
\end{align}
For small $\lambda$, $\tau$ will use the heterogeneousness of the worker-pool to better approximate the expected agreements. 

\breakcolumn

Instead of using the global chance-agreement, we compute the leave-one-out class-distribution for each item, and use these distributions to chance-correct the agreement. We call this measure $\tau$
\begin{align}
	\tau &= 1 - \frac{1}{I} \sum_i^I \frac{1 - P_i}{1 - \bar{P}_e(\Delta i)} \\
	\bar{P}_e(\Delta i) &= \sum_c p_c(\Delta i)^2 \\
	p_c(\Delta i) &= \frac{n_c - n_{ic}}{n - n_i},
\end{align}
where $\Delta i$ denote that item $i$ is not used to compute the class-distribution for $\bar{P}_e$, $n$ is the total number of annotations, $n_i$ is annotations for item $i$, $n_c$ is annotations for class $c$ and $n_{ic}$ is number of class-$c$ annotations for item $i$. The denominator and the numerator are now probabilistically independent and unbiased. We note that the elements in the sum are probabilistically \textit{dependent}, which may increase variance of the measure, but not create bias. \\

Consider the case where not all items are annotated by all annotators (we have an availability tensor $\J$). We can compute $\tau$ in a straightforward manner, and the probabilistic independence holds \textit{conditioned on the available annotations}
\begin{align}
	(P_i \perp \bar{P}_e(\Delta i) \given \J).
\end{align}

We note that $\tau$ approaches $\kappa$ with large datasize
\begin{align}
	\lim_{n \rightarrow \infty} \tau = \kappa,
\end{align}
because item $i$ will have infinitesimal influence on $p_c(\Delta i)$ with infinite data so that
\begin{align}
	\lim_{n \rightarrow \infty} p_c(\Delta i) = p_c.
\end{align}

$\tau$ is therefore a measurement similar to $\kappa$, but which eliminates the problem of probabilistic dependence, while equating $\kappa$ with large data.


\subsection{Chance Correction for Set of Workers}

\begin{figure}
	\centering
	\includegraphics[width=0.8\linewidth]{fig/ink/pdf/two_workers_disagreeing.pdf}
	\caption{
		Two example of an annotated dataset with five items and two workers.
		\textbf{Left.} The two workers agree on $\frac{1}{5}$ items. Using global class-distribution we expect agreement of $P_e = \left(\frac{4}{10}\right)^2 + \left(\frac{6}{10}\right)^2 = 0.52$ which is counter-intuitively high. Using the class-distributions of the workers we expect agreement $\bar{P}_e(w_1, w_2) = \frac{4}{5} \times 0 + \frac{1}{5} \times 1 = \frac{1}{5}$, which coincidentally matches the actual agreement (not necessarily the case). 
		\textbf{Right.} Here we have a sparse dataset with missing data. The agreement seems to be $\frac{1}{2}$, but we don't really know, because of the missing data. Using global-class distribution we expect agreement of $P_e = \left(\frac{2}{6}\right)^2 + \left(\frac{4}{6}\right)^2 = 0.56$. Using the class-distributions of the workers we expect agreement $\bar{P}_e(w_1, w_2) = \frac{2}{3} \times 0 + \frac{1}{3} \times 1 = \frac{1}{3}$.
	} \label{fig:two_disagreeing_workers}
\end{figure}

Say two workers $w_1$ and $w_2$ has annotated item $i$. In order to chance-correct their agreement, we wish to use the class-distribution. In Fleiss-kappa and $\tau$ above, we use the global class distribution for computing the chance-probability of agreement. This is, of course, not a very good approximation of the probability of these two worker agreeing (each worker may differ a lot from the "mean-worker"). When working with sparse data, it becomes increasingly important to consider which workers are annotating which item, and what the probability is of those workers agreeing by chance. \\

A more suitable measure of the probability of agreeing by chance would be to consider the empirical class-distribution of the two workers - ignoring the item itself. The empirical class-distribution of worker $w$, ignoring item $i$ is
\begin{align}
	p_c(w, \Delta i) 
		&= \frac{\sum_{j != i} \I_{wjc}}{\sum_{j != i} \I_{wj}}
		= \frac{ n_{wc} - \I_{wic} }{ n_{w} - \I_{wi} }.
\end{align}

The probability of the two workers agreeing based on their class-distributions excluding item $i$ is now
\begin{align*}
	\bar{P}_e(w_1, w_2) = \sum_c p_c(w_1, \Delta i) p_c(w_2, \Delta i).
\end{align*}

Figure \ref{fig:two_disagreeing_workers} illustrates how this measure makes intuitively more sense. \\


We now define $\mathcal{W}_i$, as the set of workers that have annotated item $i$
\begin{align}
	\mathcal{W}_i = \{ w \;:\; \I_{wi} = 1 \}, \qquad |\mathcal{W}_i| = n_i.
\end{align}

The probability of a random two workers in $\mathcal{W}$ agreeing on a new item, based on their class-distributions excluding item $i$ is
\begin{align}
	&\bar{P}_e(\mathcal{W}_i) \\
		&= \sum_{\mathclap{\substack{w_1, w_2 \in \mathcal{W}_i \\ w_2 != w_1 \\ c}}} p(w_1) p(w_2 \given w_1) p_c(w_1, \Delta i) p_c(w_2, \Delta i) \nonumber \\
		%
		&= \frac{1}{n_i (n_i - 1)} \:\:\:\: \sum_{\mathclap{\substack{w_1, w_2 \in \mathcal{W}_i \\ w_2 != w_1 \\ c}}} p_c(w_1, \Delta i) p_c(w_2, \Delta i). \nonumber
\end{align}

We can therefore compute a different version of $\tau$ which considers the specific set of worker annotating each item
\begin{align}
	\tau' &= 1 - \frac{1}{I} \sum_i^I \frac{1 - P_i}{1 - \bar{P}_e(\mathcal{W}_i)},
\end{align}
which is 1 minus the mean, chance-corrected disagreement, where the chance-correction of each item is based on the workers that annotated that item. \\

If only a subset of workers annotate each item, the interpretation of $\tau'$ is the chance-corrected probability of agreement of \textit{the specific subset of workers} observing the item. This seems intuitively more meaningful, as we chance correct by the actual workers observing the item, instead of the global worker pool, which may behave differently. \\ 




==> tex/chance_corrected_expectation.tex <==
\clearpage
\section{Bias of Chance-Corrected}

We define $O = 1 - \bar{P}_o$ and $E = 1 - \bar{P}_e$ so that
\begin{align}
	\kappa = 1 - \frac{O}{E}.
\end{align}

We use the Taylor approximation 
\begin{align}
	&\E\l[ \frac{O}{E} \r] \\
	&\approx \frac{\E[O]}{\E[E]} - \frac{\cov[O, E]}{\E[E]^2} + \frac{\var[O] \E[O]}{\E[E]^3} \nonumber
\end{align}
\inote{Consider including error term (in O-notation).}


The covariance is
\begin{align}
	&\cov[O, E] 
		= \E[(O - \E[O]) (E - \E[E])] \nonumber \\
		%
		&= \E[(1 - \bar{P}_o - \E[1 - \bar{P}_o]) (1 - \bar{P}_e - \E[1 - \bar{P}_e])] \nonumber \\
		%
		&= \E[(\E[\bar{P}_o] - \bar{P}_o) (\E[\bar{P}_e] - \bar{P}_e)] \nonumber \\
		%
		&= \E[(\bar{P}_o - \E[\bar{P}_o]) (\bar{P}_e - \E[\bar{P}_e])] \nonumber \\
		%
		&= \cov[\bar{P}_o,\bar{P}_e].
\end{align}

The covariance of $\bar{P}_o$ and $\bar{P}_e$ is
\begin{align}
	\cov[\bar{P}_o,\bar{P}_e] 
		&= \E[\bar{P}_o\bar{P}_e] - \E[\bar{P}_o]\E[\bar{P}_e] \nonumber \\
		%
		&= \E[\bar{P}_o\bar{P}_e] - PP_e \nonumber
\end{align}

The variance of $O$ is \note{It's just the variance of $\bar{P}_o$.}
\begin{align}
	\var[O] &= \E[O^2] - \E[O]^2 \\
		&= \E[(1 - \bar{P}_o)^2] - \E[1 - \bar{P}_o]^2 \nonumber \\
		&= 1 + \E[\bar{P}_o^2] -2\E[\bar{P}_o] - (1 - P)^2 \nonumber \\
		&= 1 + \E[\bar{P}_o^2] -2P - 1 - P^2 + 2P \nonumber \\
		&= \E[\bar{P}_o^2] - P^2 \nonumber
\end{align}

Error term becomes
\begin{align}
	err &= \frac{\cov[O, E]}{\E[E]^2} - \frac{\var[O] \E[O]}{\E[E]^3} \\
		&= \frac{\cov[O, E]}{(1 - \bar{P}_e)^2} - \frac{\var[O] (1 - \bar{P})}{(1 - \bar{P}_e)^3}
\end{align}


We assume that the probability of agreement is bigger than or equal to the agreement-by-chance $P \geq P_e$, so that
\begin{align}
	\cov[\bar{P}_o,\bar{P}_e] \leq \E[(\bar{P}_o - P_e) (\bar{P}_e - P_e)].
\end{align}

We expand the two random variables
\begin{align}
	\bar{P}_o &= \frac{1}{I} \sum_c \sum_i n_{ic} (n_{ic} - 1) \\
		&= \frac{1}{I} \sum_c \sum_i n_{ic}^2 - \frac{1}{I} \sum_c \sum_i n_{ic} \nonumber \\
	P_e &= \frac{1}{m^2} \sum_c \left( \sum_i n_{ic} \right)^2 \nonumber \\
		&= \frac{1}{m^2} \sum_c \sum_i n_{ic}^2 + \frac{1}{m^2} \sum_c \sum_i \sum_{j \not= i} n_{ic} n_{jc} \nonumber \\
\end{align}

The normalizers are
\begin{align}
	I &= \sum_i n_i (n_i - 1) \qquad
	m ^= \sum_i n_i
\end{align}

We let 
\begin{align}
	X &= \sum_c \left( \sum_i n_{ic} \right)^2 \\
	&= \sum_c \l( \sum_i n_{ic}^2 + 2\sum_i \sum_{j \not= i} n_{ic} n_{jc} \r) \nonumber \\
	&= \sum_c \sum_i n_{ic}^2 + 2 \sum_c \sum_i \sum_{j \not= i} n_{ic} n_{jc} \nonumber
\end{align}

 and have
\begin{align}
	&\cov[\bar{P}_o,\bar{P}_e] 
		\leq \E\l[\l(\frac{1}{I}X - P_e\r) \l(\frac{1}{m^2}X - P_e\r)\r] \nonumber \\
		%
		&= \E\l[
			\frac{1}{Im^2}X^2 - \frac{1}{m^2}XP_e
			- \frac{1}{I}XP_e + P_e^2
		\r] \nonumber \\
		%
		&= \E\l[
			\frac{1}{Im^2}X^2 - \l(\frac{1}{m^2} + \frac{1}{I}\r)XP_e + P_e^2
		\r]
\end{align}




\clearpage
\section{Expectation of Chance-Corrected}

The chance-corrected version is
\begin{align}
    \kappa = \frac{\bar{P}_o - \bar{P}_e}{1 - \bar{P}_e}
    = 1 - \frac{1 - \bar{P}_o}{1 - \bar{P}_e},
\end{align}

where 
\begin{align}
    \bar{P}_e &= \frac{1}{m^2} \sum_j m_j^2 \\
    \bar{P}_o &= \frac{1}{I} \sum_i P_i \nonumber \\
    &= \frac{1}{I} \sum_i \frac{1}{n_i (n_i - 1)} \sum_j n_{ij} (n_{ij} - 1). \nonumber
\end{align}

If we randomly remove one annotation from item $i$ we have
\begin{align}
    \E_i\left[ \frac{1 - \bar{P}_o}{1 - \bar{P}_e} \right]
        &= \sum_c \frac{n_{ic}}{n_c} \frac{1 - \hat{P}_o}{1 - \hat{P}_e}.
\end{align}

The new observed and expected probability of agreement is
\begin{align}
    &\hat{P}_e = \frac{1}{(m - 1)^2} \left( m^2 \bar{P}_e - m_c^2 + (m_c - 1)^2 \right) \nonumber \\
    &= \frac{1}{(m - 1)^2} \left( m^2 \bar{P}_e - m_c^2 + m_c^2 + 1 - 2m_c \right) \nonumber \\
    &= \frac{1}{(m - 1)^2} \left( 1 - 2m_c + m^2 \bar{P}_e \right)
\end{align}
\begin{align}
    &\hat{P}_o = \bar{P}_o \nonumber \\
    &- \frac{1}{I n_i (n_i - 1)} \sum_{j} n_{ij} (n_{ij} - 1) \nonumber \\
    &+ \frac{1}{I (n_i - 1) (n_i - 2)} \left( \sum_{j \not= c} n_{ij} (n_{ij} - 1) + (n_{ic} - 1) (n_{ic} - 2) \right) \nonumber \\
    %
    &= \bar{P}_o \nonumber \\
    &+ \frac{1}{I} \left(\frac{1}{(n_i - 1) (n_i - 2)} - \frac{1}{n_i (n_i - 1)}\right) \sum_{j \not= c} n_{ij} (n_{ij} - 1) \nonumber \\
    &+ \frac{1}{I} \left(\frac{(n_{ic} - 1) (n_{ic} - 2)}{(n_i - 1) (n_i - 2)} - \frac{n_{ic} (n_{ic} - 1)}{n_i (n_i - 1)}\right) \nonumber \\
    %
    &= \bar{P}_o \nonumber \\
    &+ \frac{1}{I} \frac{2}{(n_i - 2) (n_i - 1) n_i} (n_i - n_{ic}) \nonumber \\
    &+ \frac{1}{I} \frac{2 (n_{ic} - 1) (n_{ic} - n_i)}{(n_i - 2) (n_i - 1) n_i} \nonumber \\
    %
    &= \bar{P}_o
    + \frac{1}{I} \frac{2 (n_i - n_{ic})}{(n_i - 2) (n_i - 1) n_i} \Big( 1 - (n_{ic} - 1) \Big) \nonumber \\
    %
    &= \bar{P}_o
    + \frac{1}{I} \frac{2 (n_i - n_{ic}) ( 2 - n_{ic} )}{(n_i - 2) (n_i - 1) n_i}\nonumber
\end{align}


The expectation becomes
\begin{align}
    \E_i&\left[ \frac{1 - \bar{P}_o}{1 - \bar{P}_e} \right]
        = \sum_c \frac{n_{ic}}{n_c} 
        \frac{
            1 
            - \bar{P}_o
            + \frac{1}{I} \frac{2 (n_i - n_{ic}) ( 2 - n_{ic} )}{(n_i - 2) (n_i - 1) n_i}
        }{
            1 - \frac{1}{(m - 1)^2} \left( 1 - 2m_c + m^2 \bar{P}_e \right)
        } \nonumber \\
    %
        &= (m - 1)^2 \sum_c \frac{n_{ic}}{n_c} 
        \frac{
            1 
            - \bar{P}_o
            + \frac{1}{I} \frac{2 (n_i - n_{ic}) ( 2 - n_{ic} )}{(n_i - 2) (n_i - 1) n_i}
        }{
            (m - 1)^2 - \left( 1 - 2m_c + m^2 \bar{P}_e \right)
        } \nonumber \\
    %
        &= (m - 1)^2 \sum_c \frac{n_{ic}}{n_c} 
        \frac{
            1 
            - \bar{P}_o
            + \frac{1}{I} \frac{2 (n_i - n_{ic}) ( 2 - n_{ic} )}{(n_i - 2) (n_i - 1) n_i}
        }{
            m^2 + 1 - 2m - 1 + 2m_c - m^2 \bar{P}_e
        } \nonumber \\
    %
        &= (m - 1)^2 \sum_c \frac{n_{ic}}{n_c} 
        \frac{
            1 
            - \bar{P}_o
            + \frac{1}{I} \frac{2 (n_i - n_{ic}) ( 2 - n_{ic} )}{(n_i - 2) (n_i - 1) n_i}
        }{
            m^2 (1 - \bar{P}_e) - 2(m - m_c)
        }
\end{align}





\clearpage
\section{Expectation of Chance-Corrected 2}

The chance-corrected version is
\begin{align}
    \kappa = \frac{\bar{P}_o - \bar{P}_e}{1 - \bar{P}_e}
    = 1 - \frac{1 - \bar{P}_o}{1 - \bar{P}_e},
\end{align}

where we are going to use the \texttt{edge}-weighed version
\begin{align}
    \bar{P}_e &= \frac{1}{m^2} \sum_j m_j^2 \\
    \bar{P}_o &= \frac{1}{I} \sum_i n_i (n_i - 1) P_i \nonumber \\
    &= \frac{1}{I} \sum_i \frac{n_i (n_i - 1)}{n_i (n_i - 1)} \sum_j n_{ij} (n_{ij} - 1) \nonumber \\
    &= \frac{1}{I} \sum_i \sum_j n_{ij} (n_{ij} - 1). \nonumber
\end{align}

If we randomly remove one annotation from item $i$ we have
\begin{align}
    \E_i\left[ \frac{1 - \bar{P}_o}{1 - \bar{P}_e} \right]
        &= \sum_c \frac{n_{ic}}{n_i} \frac{1 - \hat{P}_o}{1 - \hat{P}_e}.
\end{align}

The new observed and expected probability of agreement is
\begin{align}
    &\hat{P}_e = \frac{1}{(m - 1)^2} \left( m^2 \bar{P}_e - m_c^2 + (m_c - 1)^2 \right) \nonumber \\
    &= \frac{1}{(m - 1)^2} \left( m^2 \bar{P}_e - m_c^2 + m_c^2 + 1 - 2m_c \right) \nonumber \\
    &= \frac{1}{(m - 1)^2} \left( 1 - 2m_c + m^2 \bar{P}_e \right)
\end{align}
\begin{align}
    &\hat{P}_o = \bar{P}_o
    - \frac{1}{I} \sum_{j} n_{ij} (n_{ij} - 1) \nonumber \\
    &+ \frac{1}{I} \left( \sum_{j \not= c} n_{ij} (n_{ij} - 1) + (n_{ic} - 1) (n_{ic} - 2) \right) \nonumber \\
    %
    &= \bar{P}_o
    + \frac{1}{I} \Big( (n_{ic} - 1) (n_{ic} - 2) - n_{ic} (n_{ic} - 1) \Big) \nonumber \\
    %
    &= \bar{P}_o
    + \frac{1}{I} \Big( n_{ic}^2 - n_{ic} - 2n_{ic} + 2 - n_{ic}^2 + n_{ic} \Big) \nonumber \\
    %
    &= \bar{P}_o + \frac{2}{I} (1 - n_{ic})
\end{align}

The expectation becomes
\begin{align}
    \E_i\left[ \frac{1 - \bar{P}_o}{1 - \bar{P}_e} \right]
        &= \sum_c \frac{n_{ic}}{n_i} \frac{
            1 - \bar{P}_o - \frac{2}{I} (1 - n_{ic})
        }{
            1 - \frac{1}{(m - 1)^2} \left( 1 - 2m_c + m^2 \bar{P}_e \right)
        } \nonumber \\
        %
        &= \sum_c \frac{n_{ic}}{n_i} \frac{
            1 - \bar{P}_o - \frac{2}{I} (1 - n_{ic})
        }{
            \frac{(m - 1)^2 - 1 + 2m_c - m^2 \bar{P}_e }{(m - 1)^2}
        } \nonumber \\
        %
        &= \frac{(m - 1)^2}{n_i} \sum_c n_{ic} \frac{
            1 - \bar{P}_o - \frac{2}{I} (1 - n_{ic})
        }{
           m^2 + 1 - 2m - 1 + 2m_c - m^2 \bar{P}_e
        } \nonumber \\
        %
        &= \frac{(m - 1)^2}{n_i} \sum_c n_{ic} \frac{
            1 - \bar{P}_o - \frac{2}{I} (1 - n_{ic})
        }{
           2 (m_c - m) - m^2 (1 - \bar{P}_e)
        }
\end{align}




\clearpage
\section{Expectation of Chance-Corrected 3}

The chance-corrected version is
\begin{align}
    \kappa = \frac{\bar{P}_o - \bar{P}_e}{1 - \bar{P}_e}
    = 1 - \frac{1 - \bar{P}_o}{1 - \bar{P}_e},
\end{align}

where we are going to use the \texttt{edge}-weighed version
\begin{align}
    \bar{P}_e &= \sum_c p_c^2 = \sum_c \left( \frac{m_c}{m} \right)^2 \\
        &= \frac{1}{m^2} \sum_c m_c^2 \nonumber \\
        &= \frac{1}{m^2} \sum_c \left( \sum_i n_{ic} \right)^2 \nonumber \\
    \bar{P}_o &= \frac{1}{I} \sum_i n_i (n_i - 1) P_i \nonumber \\
    &= \frac{1}{I} \sum_i \frac{n_i (n_i - 1)}{n_i (n_i - 1)} \sum_j n_{ij} (n_{ij} - 1) \nonumber \\
    &= \frac{1}{I} \sum_i \sum_j n_{ij} (n_{ij} - 1). \nonumber
\end{align}

We rewrite kappa slightly
\begin{align*}
    \frac{1 - \bar{P}_o}{1 - \bar{P}_e} 
        = m^2 \frac{1 - \bar{P}_o}{m^2 - m^2\bar{P}_e}
\end{align*}

The new observed and expected probability of agreement is
\begin{align}
    &\hat{P}_e = \frac{1}{(m - 1)^2} \left( m^2 \bar{P}_e - m_c^2 + (m_c - 1)^2 \right) \nonumber \\
    &= \frac{1}{(m - 1)^2} \left( m^2 \bar{P}_e - m_c^2 + m_c^2 + 1 - 2m_c \right) \nonumber \\
    &= \frac{1}{(m - 1)^2} \left( 1 - 2m_c + m^2 \bar{P}_e \right)
\end{align}

So that
\begin{align}
    \hat{P}_e (m - 1)^2 = 1 - 2m_c + m^2 \bar{P}_e
\end{align}
\begin{align}
    m^2 \bar{P}_e = \hat{P}_e (m - 1)^2 - 1 + 2m_c
\end{align}

\begin{align}
    &\hat{P}_o = \bar{P}_o
    - \frac{1}{I} \sum_{j} n_{ij} (n_{ij} - 1) \nonumber \\
    &+ \frac{1}{I} \left( \sum_{j \not= c} n_{ij} (n_{ij} - 1) + (n_{ic} - 1) (n_{ic} - 2) \right) \nonumber \\
    %
    &= \bar{P}_o
    + \frac{1}{I} \Big( (n_{ic} - 1) (n_{ic} - 2) - n_{ic} (n_{ic} - 1) \Big) \nonumber \\
    %
    &= \bar{P}_o
    + \frac{1}{I} \Big( n_{ic}^2 - n_{ic} - 2n_{ic} + 2 - n_{ic}^2 + n_{ic} \Big) \nonumber \\
    %
    &= \bar{P}_o + \frac{2}{I} (1 - n_{ic})
\end{align}

So that
\begin{align}
    \bar{P}_o = \hat{P}_o + \frac{2}{I} (n_{ic} - 1)
\end{align}


We now compute the following statistic
\begin{align}
    X = m^2 \frac{1 - \hat{P}_o}{m^2 - m^2\hat{P}_e} + \sum_c \frac{n_{ic}}{n_i} \frac{ \frac{2}{I} (n_{ic} - 1) }{ m^2 - m^2 \hat{P}_e }
\end{align}

In expectation this statistic will have the value of
\begin{align}
    &\E_i[X] \nonumber \\
         &= \sum_c \frac{n_{ic}}{n_i} m^2 \frac{1 - \hat{P}_o}{m^2 - m^2\hat{P}_e} \nonumber \\
         %
         &= \frac{m^2}{n_i} \sum_c n_{ic} \frac{1 - \hat{P}_o}{m^2 - m^2\hat{P}_e}
\end{align}




\clearpage
\section{Expectation of Chance-Corrected 4}

The chance-corrected version is
\begin{align}
    \kappa = \frac{\bar{P}_o - \bar{P}_e}{1 - \bar{P}_e}
    = 1 - \frac{1 - \bar{P}_o}{1 - \bar{P}_e},
\end{align}

where we are going to use the \texttt{edge}-weighed version
\begin{align}
    \bar{P}_e &= \sum_c p_c^2 = \sum_c \left( \frac{m_c}{m} \right)^2 \\
        &= \frac{1}{m^2} \sum_c m_c^2 \nonumber \\
        &= \frac{1}{m^2} \sum_c \left( \sum_i n_{ic} \right)^2 \nonumber \\
    \bar{P}_o &= \frac{1}{I} \sum_i n_i (n_i - 1) P_i \nonumber \\
    &= \frac{1}{I} \sum_i \frac{n_i (n_i - 1)}{n_i (n_i - 1)} \sum_j n_{ij} (n_{ij} - 1) \nonumber \\
    &= \frac{1}{I} \sum_i \sum_j n_{ij} (n_{ij} - 1). \nonumber
\end{align}


We now randomly select an annotation which we remove. The sampling can be performed by first sampling a category by its size, and them sampling an item, by their counts of the selected category.
\begin{align}
    &\E\left[ \frac{1 - \bar{P}_o}{1 - \bar{P}_e} \right]
        = \sum_c \frac{m_c}{m} \sum_i \frac{n_{ic}}{m_c} \frac{1 - \hat{P}_o}{1 - \hat{P}_e} \\
        %
        &= \sum_c \frac{m_c}{m} \sum_i \frac{n_{ic}}{m_c} \frac{1 - \hat{P}_o}{1 - \hat{P}_e} \nonumber 
\end{align}


The new expected probability of agreement is
\begin{align}
    &\hat{P}_e = \frac{1}{(m - 1)^2} \left( m^2 \bar{P}_e - m_c^2 + (m_c - 1)^2 \right) \nonumber \\
    &= \frac{1}{(m - 1)^2} \left( m^2 \bar{P}_e - m_c^2 + m_c^2 + 1 - 2m_c \right) \nonumber \\
    &= \frac{1}{(m - 1)^2} \left( 1 - 2m_c + m^2 \bar{P}_e \right)
\end{align}

So that
\begin{align}
    \hat{P}_e (m - 1)^2 &= 1 - 2m_c + m^2 \bar{P}_e \\
    m^2 \bar{P}_e &= \hat{P}_e (m - 1)^2 - 1 + 2m_c \\
    \bar{P}_e &= \frac{\hat{P}_e (m - 1)^2 - 1 + 2m_c}{m^2} \\
    \bar{P}_e &= \frac{\hat{P}_e (m - 1)^2 - 1 + 2m_c}{m^2}
\end{align}

If we use the numbers after removal we have
\begin{align}
 \bar{P}_e &= \frac{\hat{P}_e ((\hat{m} + 1) - 1)^2 - 1 + 2(\hat{m}_c + 1)}{(\hat{m} + 1)^2} \\
 \bar{P}_e &= \frac{\hat{P}_e \hat{m}^2 + 1 + 2\hat{m}_c}{(\hat{m} + 1)^2}
\end{align}

The new observed probability of agreement is
\begin{align}
    &\hat{P}_o = \bar{P}_o
    - \frac{1}{I} \sum_{j} n_{ij} (n_{ij} - 1) \nonumber \\
    &+ \frac{1}{I} \left( \sum_{j \not= c} n_{ij} (n_{ij} - 1) + (n_{ic} - 1) (n_{ic} - 2) \right) \nonumber \\
    %
    &= \bar{P}_o
    + \frac{1}{I} \Big( (n_{ic} - 1) (n_{ic} - 2) - n_{ic} (n_{ic} - 1) \Big) \nonumber \\
    %
    &= \bar{P}_o
    + \frac{1}{I} \Big( n_{ic}^2 - n_{ic} - 2n_{ic} + 2 - n_{ic}^2 + n_{ic} \Big) \nonumber \\
    %
    &= \bar{P}_o + \frac{2}{I} (1 - n_{ic})
\end{align}

So that
\begin{align}
    \bar{P}_o = \hat{P}_o + \frac{2}{I} (n_{ic} - 1)
\end{align}


Backwards
\begin{align}
	& \E \left[ \frac{
		1 - \hat{P}_o + \frac{2}{I} (n_{ic} - 1)
	}{
		1 - \frac{\hat{P}_e \hat{m}^2 + 1 + 2\hat{m}_c}{(\hat{m} + 1)^2}
	} \right] \\
	&= \frac{1 - \bar{P}_o}{1 - \bar{P}_e} \nonumber
\end{align}



\clearpage
\section{Expectation of Chance-Corrected 4b}


The covariance of $\bar{P}_o$ and $\bar{P}_e$ is
\begin{align}
	&\cov[\bar{P}_o,\bar{P}_e] 
		= \E[(\bar{P}_o - \E[\bar{P}_o]) (\bar{P}_e - \E[\bar{P}_e])] \\
		%
		&= \E[(\bar{P}_o - P) (\bar{P}_e - \sum_c p_c^2)] \nonumber \\
		%
		&= \E\l[
			\l(\frac{1}{I} \sum_i \sum_j n_{ij} (n_{ij} - 1) - P\r) 
			\l(\frac{1}{m^2} \sum_c \left( \sum_i n_{ic} \right)^2 - P_e\r)
		\r] \nonumber \\
		%
		&= 
		-\E\l[ \frac{1}{I} \sum_i \sum_j n_{ij} (n_{ij} - 1) \r] P_e
		+\E\l[ \frac{1}{I} \sum_i \sum_j n_{ij} (n_{ij} - 1) \frac{1}{m^2} \sum_c \left( \sum_i n_{ic} \right)^2 \r]
		-\E\l[ \frac{1}{m^2} \sum_c \left( \sum_i n_{ic} \right)^2 \r] P
		+ P P_e \nonumber \\
		%
		&= 
		-P P_e
		+\E\l[ \frac{1}{Im^2} \sum_c \sum_i n_{ic} (n_{ic} - 1) \sum_{c'} \left( \sum_i n_{ic'} \right)^2 \r]
		-P_e P
		+ P P_e \nonumber \\
		%
		&= 
		\frac{1}{Im^2} \sum_c \sum_{c'} \E\l[ \left( \sum_i n_{ic'} \right)^2 \sum_i n_{ic} (n_{ic} - 1) \r]
		-P_e P \nonumber \\
		%
		&= 
		\frac{1}{Im^2} \sum_c \sum_{c'} \E\l[ \sum_i \sum_j \sum_{\ell} n_{ic'} n_{jc'} n_{\ell c} (n_{\ell c} - 1) \r]
		-P_e P \nonumber \\
		%
		&= 
		\frac{1}{Im^2} \sum_c \sum_{c'} \sum_i \sum_j \sum_{\ell} \E\l[ n_{ic'} n_{jc'} n_{\ell c} (n_{\ell c} - 1) \r]
		-P_e P \nonumber \\
		%
		&= 
		\frac{1}{Im^2} \sum_c \sum_{c'} \sum_i \E\l[ n_{i c}^3 (n_{i c} - 1) \r]
		-P_e P
\end{align}

We note that
\begin{align}
	\E[n_{ic}] &= \sum_i^n (1 - d)^i \sum_j^i p_c^j j \nonumber \\
	\E[n_{ic}^2] &= \sum_i^n (1 - d)^i \sum_j^i p_c^j j^2 \nonumber \\
	\E[n_{ic} (n_{ic} - 1)] &= \sum_i^n (1 - d)^i \sum_j^i p_c^j j (j - 1) \nonumber \\
	\E[n_{ic}^2 (n_{ic} - 1)] &= \sum_i^n (1 - d)^i \sum_j^i p_c^j j^2 (j-1) \nonumber \\
	\E[n_{ic}^3 (n_{ic} - 1)] &= \sum_i^n (1 - d)^i \sum_j^i p_c^j j^3 (j-1) \nonumber \\
\end{align}
where $d$ is the ratio of deleted annotations.

\begin{align}
    \kappa = \frac{\bar{P}_o - \bar{P}_e}{1 - \bar{P}_e}
    = 1 - \frac{1 - \bar{P}_o}{1 - \bar{P}_e},
\end{align}


\begin{align}
	\E \l[ \frac{1 - \bar{P}_o}{1 - \bar{P}_e} \r] 
		\approx \frac{ \E \l[  1 - \bar{P}_o \r] }{ \E \l[  1 - \bar{P}_e \r] } - \frac{cov}{mean}
\end{align}



\clearpage
\section{Expectation of Chance-Corrected 4c}

\inote{
\begin{itemize}
	\item Compute estimation of $P_o$
	\item Use class distribution to resample class frequencies (and subsample class distributions)
	\item Numerically compute distribution of $P_e$
	\item Compute chance-corrected kappa, while numerically integrating over $P_e$
\end{itemize}
}




We have an item with $n$ annotations in annotation vector $\vn$. 
We now remove $d$ random annotations in deletion vector $\vd$. The probability of $\vd$ is
\begin{align}
	\vd &= \vn - \veta \\
	p(\vd \given \vn) 
		&= \prod_c {\evn_c \choose \evd_c}
		\times \frac{1}{(n - d + 1)^{d+1}} \nonumber \\ 
		&\times \prod_c (\evn_c-\evd_c+1)^{(\evd_c + 1)} \nonumber \\
	%
		&= 
		\frac{1}{(n - d + 1)^{d+1}} \times \nonumber \\
		&\prod_c {\evn_c \choose \evd_c} (\evn_c-\evd_c+1)^{(\evd_c + 1)} \nonumber \\ 
\end{align}

The prior on any vector is
\begin{align}
	p(\vn) = \prod_c \evn_c^{\evp_c}.
\end{align}

The inverse probability is
\begin{align}
	p(\vn \given \vd) = \frac{p(\vd \given \vn) \; p(\vn)}{\sum_{\vn' \in \mathcal{D}_n^C} p(\vd \given \vn') \; p(\vn')} 
\end{align}


The probability of the remaining annotations being vector $\veta$ is
\begin{align}
	p(\veta \given \vn) = \prod_c (\eveta_c+1)^{(\evn_c - \eveta_c + 1)} \times \frac{1}{(n - d)^{d+1}}
\end{align}
where we use the rising factorial 
\begin{align}
	x^{(n)} = x(x+1) ... (x + n - 1)
\end{align}

We have an item, where $d$ annotations have been removed. 

We have an item, where one annotation has been removed. 
The probability of class $c$ having one annotation removed is
\begin{align}
	p_r(c \given \hat{\vn}) 
		&= \frac{\hat{\vn}_c + 1}{\vone^{\top} \hat{\vn}} \times \frac{1}{\sum_{j} \frac{\hat{\vn}_j + 1}{\vone^{\top} \hat{\vn}}} \\
		&= \frac{\hat{\vn}_c + 1}{\sum_{j} \hat{\vn}_j + 1}
		= \frac{\hat{\vn}_c + 1}{\vone^{\top} \hat{\vn} + C}.
\end{align}



\clearpage
\section{Expectation of Chance-Corrected 5}

The chance-corrected version is
\begin{align}
    \kappa = \frac{\bar{P}_o - \bar{P}_e}{1 - \bar{P}_e}
    = 1 - \frac{1 - \bar{P}_o}{1 - \bar{P}_e},
\end{align}

where we are going to use the \texttt{edge}-weighed version
\begin{align}
    \bar{P}_e &= \sum_c p_c^2 = \sum_c \left( \frac{m_c}{m} \right)^2 \\
        &= \frac{1}{m^2} \sum_c m_c^2 \nonumber \\
        &= \frac{1}{m^2} \sum_c \left( \sum_i n_{ic} \right)^2 \nonumber \\
    \bar{P}_o &= \frac{1}{I} \sum_i n_i (n_i - 1) P_i \nonumber \\
    &= \frac{1}{I} \sum_i \frac{n_i (n_i - 1)}{n_i (n_i - 1)} \sum_j n_{ij} (n_{ij} - 1) \nonumber \\
    &= \frac{1}{I} \sum_i \sum_j n_{ij} (n_{ij} - 1). \nonumber
\end{align}


For an item with 2 annotations, the expected number of edges $\tau$ in class $c$ is
\begin{align}
    \E_2[\texttt{edges}, c] = \tau_2(c) = p_c^2,
\end{align}
and the total number of edges
\begin{align}
    \E_2[\texttt{edges}] = \sum_c \tau_2(c).
\end{align}

For an item with $n$ annotations, the expected number of edges in class $c$ is
\begin{align}
    \tau_n(c) = p_c^n \frac{n(n - 1)}{2} + (1 - p_c) \tau_{n-1}(c). \nonumber
\end{align}

The expected agreement for an item with $n$ annotations is
\begin{align}
    \E_n[P] = \frac{2}{n (n - 1)} \sum_c \tau_{n}(c).
\end{align}

The expected agreement by change over the dataset is
\begin{align}
    \E_{\mathcal{D}}[P] = \frac{1}{I} \sum_i \frac{n_i (n_i - 1)}{2} \E_{n_i}[P].
\end{align}

Which can be simplified to be
\begin{align}
    \frac{1}{I} \sum_n^{\max_i n_i} \theta_n \frac{n (n - 1)}{2} \E_n[P],
\end{align}
where $\theta_n$ is the number of items in a dataset with $n$ annotations.


\subsection{Full Annotation}

Let's assume that all items have exactly $n$ annotations. The expected agreement becomes
\begin{align}
     \E_{\mathcal{D}}[P] &= \frac{1}{I} \theta_n \frac{n (n - 1)}{2} \E_n[P] \nonumber \\
        &= \frac{1}{I} I \E_n[P] = \E_n[P]
\end{align}

\inote{We need to show that the above becomes the expected agreement from Fleiss, when we have a full dataset.}
\inote{Also we might want to show that the expectation of the whole thing remains the same when removing annotations?}

\vspace{2cm}

We will enumerate all possible combinations of $n$ annotations into $C$ categories, and determine the ... 
\begin{align}
	\E_n[P]&= \sum_{ \vn \in \mathcal{P}^n_C } 
			 p(\vn) \frac{1}{N} \sum_c \frac{\evn_c(\evn_c - 1)}{2} \nonumber
\end{align}

The probability of $\evn_c$ is (sample from a binomial distribution)
\begin{align}
	p(\evn_c) = {n \choose \evn_c} p_c^{\evn_c} (1 - p_c)^{n - \evn_c}.
\end{align}

So we have
\begin{align}
	\E_n[P]&= \frac{1}{N} \sum_{ \vn \in \mathcal{P}^n_C } 
		p(\vn) \sum_c \frac{\evn_c(\evn_c - 1)}{2} \nonumber \\
		%
		&= \frac{1}{N} 
		\sum_{c} \sum_{\evn_c}^n p(\evn_c)
		\frac{\evn_c(\evn_c - 1)}{2} \nonumber
\end{align}















